Magnetic field measurements on the mini-ICAL detector using Hall probes

The magnetised 51 kton Iron Calorimeter (ICAL) detector proposed to be built at INO is designed with a focus on detecting 1-20 GeV muons. The magnetic field will enable the measurement of the momentum of the $\mu^-$ and $\mu^+$ generated from the charge current interactions of $\nu_\mu$ and $\bar\nu_\mu$ separately within iron in the detector, thus permitting the determination of the neutrino mass ordering/hierarchy, among other important goals of ICAL. Hence it is important to determine the magnetic field as accurately as possible. The mini-ICAL detector is an 85-ton prototype of ICAL, which is operational at Madurai in South India. We describe here the first measurement of the magnetic field in mini-ICAL using Hall sensor PCBs. A set-up developed to calibrate the Hall probe sensors using an electromagnet. The readout system has been designed using an Arduino Nano board for selection of channels of Hall probes mounted on the PCB and to convert the analog voltage to a digital output. The magnetic field has been measured in the small gaps (provided for the purpose) between iron plates in the top layer of mini-ICAL as well as in the air just outside the detector. A precision of better than 3% was obtained, with a sensitivity down to about 0.03 kGauss when measuring the small fringe fields outside the detector.

==> author <==
Honey (HBNI, IMSc, TIFR, India), B. Satyanarayana (TIFR), R. Shinde (TIFR), V.M. Datar (IMSc), D. Indumathi (IMSc, HBNI), Ram K V Thulasi (TIFR), N. Dalal (BARC), S. Prabhakar (BARC), S. Ajith (BARC), Sourabh Pathak (BARC), Sandip Patel (BARC)

The magnetised 51 kton Iron Calorimeter (ICAL) detector proposed to be built at INO is designed with a focus on detecting 1-20 GeV muons. The magnetic field will enable the measurement of the momentum of the \mu^- and \mu^+ generated from the charge current interactions of \nu_\mu and \bar\nu_\mu separately within iron in the detector, thus permitting the determination of the neutrino mass ordering/hierarchy, among other important goals of ICAL. Hence it is important to determine the magnetic field as accurately as possible. The mini-ICAL detector is an 85-ton prototype of ICAL, which is operational at Madurai in South India. We describe here the first measurement of the magnetic field in mini-ICAL using Hall sensor PCBs. A set-up developed to calibrate the Hall probe sensors using an electromagnet. The readout system has been designed using an Arduino Nano board for selection of channels of Hall probes mounted on the PCB and to convert the analog voltage to a digital output. The magnetic field has been measured in the small gaps (provided for the purpose) between iron plates in the top layer of mini-ICAL as well as in the air just outside the detector. A precision of better than 3% was obtained, with a sensitivity down to about 0.03 kGauss when measuring the small fringe fields outside the detector.


